Nested Named Entity Recognition with Partially-Observed TreeCRFs

Named entity recognition (NER) is a well-studied task in natural language processing. However, the widely-used sequence labeling framework is difficult to detect entities with nested structures. In this work, we view nested NER as constituency parsing with partially-observed trees and model it with partially-observed TreeCRFs. Specifically, we view all labeled entity spans as observed nodes in a constituency tree, and other spans as latent nodes. With the TreeCRF we achieve a uniform way to jointly model the observed and the latent nodes. To compute the probability of partial trees with partial marginalization, we propose a variant of the Inside algorithm, the \textsc{Masked Inside} algorithm, that supports different inference operations for different nodes (evaluation for the observed, marginalization for the latent, and rejection for nodes incompatible with the observed) with efficient parallelized implementation, thus significantly speeding up training and inference. Experiments show that our approach achieves the state-of-the-art (SOTA) F1 scores on the ACE2004, ACE2005 dataset, and shows comparable performance to SOTA models on the GENIA dataset. Our approach is implemented at: \url{https://github.com/FranxYao/Partially-Observed-TreeCRFs}.

==> 035inside.tex <==
% \begin{algorithm}[t]
%   \caption{\label{alg:partial_summation} Partial Marginalization}
%   \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
%   \Input{Scores $s$, partial tree $T$}
%   \Output{}
%   \BlankLine
%   \For{$k \gets 1$ to $N$}                    
%     \State {$\beta_{iik}$}
%   \EndFor
%   mask = [length, length, label size + latent size]
  
%   \If{span[i,j] is entity}{ mask[i,j,label] = 1 other  mask[i,j,label]  = 0 }
% \end{algorithm}	



\begin{algorithm}[t!]
  \small
  \caption{\label{alg:inside} \textsc{Inside}}
  \begin{algorithmic}[1]
  
  \State Input: Scores $s$
  \For{$i \gets 1$ to $n$}    
    \State $\beta[i, i, k] = \exp(s_{iik})$ \label{alg:line_masked_leaf} 
  \EndFor
  \For{$d \gets 1$ to $n - 1$}       
    \State \begin{varwidth}[h]{\linewidth} 
      Parallelization on $i$, tensor operation on $l, k, k_1, k_2$ \label{alg:line_parallel} \par
        \hskip\algorithmicindent  $1 \le i \le n - d$; $\;\; j = i + d$;  $\;\; k, k_1, k_2 \in \{1, ..., |\mathcal{L}|\}$
      \end{varwidth}
    % \State $\beta[i, j] = (M[i, j] \exp{s_{i, j}}) \sum_{i \le r < j} \exp(\beta[i, r] + \beta[r + 1, j])$
    \State \begin{varwidth}[h]{\linewidth} \label{alg:line_masked_sum}
      $\beta[i, j, k] =  \exp(s_{i j k}) \; \cdot$  \par
        \hskip\algorithmicindent $\sum_{l = i}^{j - 1} \sum_{k_1, k_2 \in \mathcal{L}} \beta[i, l, k_1] \beta[l + 1, j, k_2]$
      \end{varwidth}
  \EndFor

  \State Return: $s(T) = \log(\sum_{k \in \mathcal{L}} \beta[1, n, k])$
  
\end{algorithmic}
\end{algorithm}



==> 0416_latent_analysis_result.tex <==
\begin{table}[t!]
	\small
	\begin{center}
		\begin{tabular}{@{} l ccccccc @{}}
			\toprule
			& PER & LOC & ORG & GPE & FAC & VEH & WEA \\
			\hline
PER & 12:115 & 12:11 & 11:5 & 12:11 & 9:16,11:16 & 12:3,13:3 & 7:1,9:1,11:1 \\ 
LOC & 8:3,9:3 & 12:13 & 13:5 & 12:2 & 12:2 & 5:1,7:1,8:1,9:1,13:1 &  \\ 
ORG & 10:59 & 11:1 & 11:57 & 12:2 & 7:7 & 11:2,12:2,13:2 &  \\ 
GPE & 10:57 & 13:5 & 9:19 & 11:16 & 11:20 & 11:6 & 10:1 \\ 
FAC & 12:30 & 9:4 &  & 10:3 & 9:10 &  &  \\ 
VEH & 7:18 & 11:2 &  & 11:2 & 10:2 & 12:18 &  \\ 
WEA & 9:6,10:6 &  &  & 11:2 &  & 13:1 & 11:6 \\ 
			\bottomrule
		\end{tabular}		
	\end{center}
	\caption{\label{tab:error} Latent distribution on ACE2005.} 
\end{table}



\begin{table}[t!]
	\small
	\begin{center}
		\begin{tabular}{@{} l ccccccc @{}}
			\toprule
			& PER & LOC & ORG & GPE & FAC & VEH & WEA \\
			\hline
PER & 12:871 & 7:33 & 12:98 & 9:64 & 10:47 & 12:58 & 12:17 \\ 
LOC & 12:97 & 13:48 & 12:11 & 12:27 & 7:44 & 12:18 & 9:1,12:1 \\ 
ORG & 12:354 & 13:17 & 9:231 & 9:23 & 9:27 & 7:18 & 12:18 \\ 
GPE & 7:387 & 7:85 & 12:140 & 9:201 & 9:130 & 7:24 & 9:15 \\ 
FAC & 12:72 & 8:2,12:2 & 12:15 & 12:4 & 9:53 & 7:3,12:3 &  \\ 
VEH & 12:37 &  & 12:4 & 7:14 & 7:3,9:3,12:3 & 12:72 & 9:5 \\ 
WEA & 12:39 &  & 12:3 & 9:19 & 9:20 & 7:4 & 12:59 \\
			\bottomrule
		\end{tabular}		
	\end{center}
	\caption{\label{tab:error} Latent distribution on ACE2005.} 
\end{table}

\begin{table}[t!]
	\small
	\begin{center}
		\begin{tabular}{@{} l ccccccc @{}}
			\toprule
			& PER & LOC & ORG & GPE & FAC & VEH & WEA \\
			\hline
			PER & 12:871 & 7:33 & 12:98 & 9:64 & 10:47 & 12:58 & 12:17 \\ 
			LOC & 12:97 & 13:48 & 12:11 & 12:27 & 7:44 & 12:18 &  \\ 
			ORG & 12:354 & 13:17 & 9:231 & 9:23 & 9:27 & 7:18 & 12:18 \\ 
			GPE & 7:387 & 7:85 & 12:140 & 9:201 & 9:130 & 7:24 & 9:15 \\ 
			FAC & 12:72 &  & 12:15 &  & 9:53 &  &  \\ 
			VEH & 12:37 &  &  & 7:14 &  & 12:72 &  \\ 
			WEA & 12:39 &  &  & 9:19 & 9:20 &  & 12:59 \\ 
			\bottomrule
		\end{tabular}		
	\end{center}
	\caption{\label{tab:error} Latent distribution on ACE2005.} 
\end{table}


\begin{table}[t!]
	\small
	\begin{center}
		\begin{tabular}{@{} l ccccccc @{}}
			\toprule
			& PER & LOC & ORG & GPE & FAC & VEH & WEA \\
			\hline
PER & 7:737,8:481,9:672,10:721,11:525,12:871,13:443 & 7:33,9:32,11:20,12:17,13:26 & 7:67,8:62,9:67,12:98 & 7:46,9:64,11:41,12:46 & 7:30,9:45,10:47,11:26,12:27,13:29 & 7:34,9:35,11:32,12:58 & 10:13,11:11,12:17,13:9 \\ 
LOC & 7:52,10:51,12:97 & 7:39,9:26,10:33,12:36,13:48 & 10:8,11:9,12:11 & 7:23,8:14,9:23,11:14,12:27 & 7:44,9:38,10:25,11:25,12:37 & 7:14,9:10,12:18 & 9:1,12:1 \\ 
ORG & 7:274,8:209,9:263,10:218,11:191,12:354 & 9:9,11:9,13:17 & 9:231,12:149 & 7:21,9:23,10:13,11:14,13:18 & 9:27,12:15 & 7:18,12:10,13:10 & 11:11,12:18 \\ 
GPE & 7:387,8:273,9:280,10:335,11:227,12:311,13:220 & 7:85,10:56,12:45,13:47 & 7:113,9:77,10:116,12:140 & 7:189,8:102,9:201,10:146,11:172,12:153 & 7:103,8:71,9:130,10:104,11:94,12:89 & 7:24,12:17 & 7:8,9:15,12:12,13:8 \\ 
FAC & 9:41,12:72 & 8:2,9:1,12:2,13:1 & 11:8,12:15 & 4:2,9:2,12:4 & 7:30,9:53,10:43,11:27 & 7:3,12:3 &  \\ 
VEH & 7:29,9:31,10:25,12:37 &  & 7:2,8:2,12:4 & 7:14,8:10,11:9 & 7:3,9:3,12:3 & 7:55,9:43,12:72 & 9:5 \\ 
WEA & 9:34,12:39 &  & 8:2,9:2,12:3,13:2 & 9:19,13:10 & 9:20 & 7:4,13:3 & 7:47,9:53,10:35,11:53,12:59 \\ 
			\bottomrule
		\end{tabular}		
	\end{center}
	\caption{\label{tab:error} Latent distribution on ACE2005.} 
\end{table}

==> 046ablation.tex <==
\begin{table*}[h!]
  \begin{center}
    \begin{tabular}{@{} l c c c c c c @{}}
      \toprule
         & \multicolumn{3}{c}{ACE2004} 	& \multicolumn{3}{c}{ACE2005}  \\ 
      % \cline{2-7}
      Method & P & R & F1 & P & R & F1 \\
      \hline
      PO-TreeCRFs base & 86.7 & 86.5 & 86.6 &  83.0 & 87.2 & 85.0 \\
      \hline
      Change Biaffine to Bilinear & 86.0 & 86.7 & 86.4 & 83.0 & 86.5 & 84.7   \\
      % W/o. biaffine & 86.0 & 86.7 & 86.4 & 83.0 & 86.5 & 84.7   \\
      % - biaffine &  & & & & & \\
      % deep-biaffine  &  & & & & & \\
    %  W/o. dropout & 84.7 & 86.6 & 85.7 & 81.5 & 88.1 & 84.7 \\
      % Change decoding to Margin & 86.2 & 86.4 & 86.3 & 83.7 & 86.4 & 85.0 \\
      % argmax (use this) &  & & & & & \\
      % entropy (no use) &  & & & & & \\
      % state dropout (no use) &  & & & & & \\
      W/o. TreeCRF & 84.4 & 85.4 & 84.9 & 82.0 & 86.4 & 84.1 \\ 
      W/o. Potential Normalization & 86.0 & 85.3 & 85.7 & 82.7 & 86.2 & 84.4 \\ 
      W/o. Structure Smoothing & 86.1 & 86.4 & 86.2 & 83.5 & 85.8 & 84.6 \\
      \bottomrule
    \end{tabular}		
  \end{center}
  \caption{Ablation Study} 
  \label{exp:ablation_study}
\end{table*}

% TODO: add model hyperparams. 

==> 049model_params.tex <==
\begin{table}
  \begin{center}
    \begin{tabular}{@{} l c c  @{}}
      \toprule
        & ACE2004	& ACE2005  \\ 
      % \cline{2-7}
      \hline
      deep biaffine \# layers & 2 & 2 \\ 
      learning rate & & \\ 
      dropout & 0.x & 0.x \\ 
      decode method & argmax & argmax \\
      label smoothing (useful) & 0.9x & 0.9x \\
      \bottomrule
    \end{tabular}		
  \end{center}
  \caption{Ablation Test} 
  \label{result}
\end{table}
